Dual Quaternion-Based Visual Servoing for Grasping Moving Objects

This paper presents a new dual quaternion-based formulation for pose-based visual servoing. Extending our previous work on local contact moment (LoCoMo) based grasp planning, we demonstrate grasping of arbitrarily moving objects in 3D space. Instead of using the conventional axis-angle parameterization, dual quaternions allow designing the visual servoing task in a more compact manner and provide robustness to manipulator singularities. Given an object point cloud, LoCoMo generates a ranked list of grasp and pre-grasp poses, which are used as desired poses for visual servoing. Whenever the object moves (tracked by visual marker tracking), the desired pose updates automatically. For this, capitalising on the dual quaternion spatial distance error, we propose a dynamic grasp re-ranking metric to select the best feasible grasp for the moving object. This allows the robot to readily track and grasp arbitrarily moving objects. In addition, we also explore the robot null-space with our controller to avoid joint limits so as to achieve smooth trajectories while following moving objects. We evaluate the performance of the proposed visual servoing by conducting simulation experiments of grasping various objects using a 7-axis robot fitted with a 2-finger gripper. Obtained results demonstrate the efficiency of our proposed visual servoing.

==> sections/stability.tex <==

\subsection{Stability Proof}

In this section we present the stability proof for closed-loop system proposed in equation \eqref{eq:jointController} in the previous section. First, let $\dq z(t)=\quat{z_{P}}+\varepsilon\quat{z_{D}}=1-\dq e$ describe the error, with its dynamics being $\dq{\dot z}=-\dq{\dot e}$. Therefore, as  $\dq z \rightarrow 0$ then $\dq e \rightarrow 1$ and $\dq x_c\rightarrow\dq x_d$. Henceforth, we can define a Lyapunov candidate function
\begin{equation}
    V(\dq z(t) ) = V_1(\quat{z_{P}}(t))+V_2(\quat {z_{D}}(t)) \label{eq:lypu_candidate}
\end{equation}
where, $V_1(\quat {z_{P}}(t))=\norm{ \quat{z_{P}}}^2$ and $V_2(\quat {z_{D}}(t))=\norm{ \quat{z_{D}}}^2$ are both positive definite functions.
Furthermore, we note that the error, which can be expanded as in \eqref{eq:quatset} and \eqref{eq:dq_set} to $\dq e = (\eta_P + \quat{\mu_P})+\dual (\eta_D + \quat{\mu_D})$, must be a unit dual quaternion. Then it directly follows that $\eta_P^2+\norm{\quat{\mu_P}}^2 = 1$. Thus,
\begin{equation}
\begin{gathered}
    V_1(\quat {z_{P}}(t))= \norm{1-\quat e}^2 = 2(1-\eta_P)\\
    V_2(\quat {z_{D}}(t))= \norm{\quat e}^2 =\eta_D^2+ \norm{\quat \mu_D}^2  \label{eq:lypu_candidate_parts}
\end{gathered}
\end{equation}
%
By taking the first order derivative of \eqref{eq:lypu_candidate_parts} we will have 
\begin{equation}
\begin{gathered}
     \dot{V_1}(\quat {z_{P}}(t))= -2\dot \eta_P\\
     \dot{V_2}(\quat {z_{D}}(t))= 2\eta_D\dot{\eta_D}+ 2\langle \quat \mu_D,\quat{\dot\mu_D}\rangle \label{eq:lypu_candidate_parts_derivative}
\end{gathered}
\end{equation}
%
where the individual derivatives stem directly from the definitions in \eqref{eq:inner_product}, \eqref{eq:vec_product} and \eqref{eq:twist} as in \cite{KUSSABA2017}. That is, 
\begin{equation}
\begin{gathered}
     \dot \eta_P = -\frac{\langle \quat {h_P}, \quat{\mu_P} \rangle }{2}\\
     \dot \eta_D = -\frac{\langle \quat {h_P}, \quat{\mu_D} \rangle + \langle \quat {h_D}, \quat{\mu_P} \rangle }{2}\\
     \dot \mu_D = \frac{\eta_D \quat {h_P}+\eta_P\quat{h_D}+\quat{h_P}\times \quat{\mu_D}+\quat{h_D}\times \quat{\mu_P}}{2} \label{eq:element_derivative}
\end{gathered}
\end{equation}
%
with $\dq h = \quat{h_P}+\dual \quat{h_D}$ being our closed loop system dynamics stemming from \eqref{eq:twist} and \eqref{eq:DQ_log}, that is, $\quat{h_P}=-\frac{1}{2}K\phi_e \quat n_e$ and $\quat{h_D}=-\frac{1}{2}K \quat p_e$. Hence, we can rewrite \eqref{eq:element_derivative} as
\begin{equation}
\begin{gathered}
     \dot{V_1}(\quat {z_{P}}(t))= \langle \quat {h_P}, \quat{\mu_P} \rangle\\
     \dot{V_2}(\quat {z_{D}}(t))= \langle (\eta_P \quat {\mu_D}-\eta_D\quat{\mu_P}+ \quat{\mu_P}\times \quat{\mu_D}),\quat {h_D}\rangle \label{eq:lypu_candidate_parts2}
\end{gathered}
\end{equation}
which from \eqref{eq:rotation_quat} and as in \cite{KUSSABA2017} yields 
\begin{equation}
    \dot{V_1}(\quat {z_{P}}(t))= \langle -\frac{1}{2}K\phi_e\quat n_e, \quat{\mu_P} \rangle = -K\langle \frac{1}{2}\phi_e\quat n_e, \text{sin}\left (\frac{1}{2}\phi_e\right )\quat n_e \rangle  \nonumber
\end{equation}
\begin{multline}
    \dot{V_2}(\quat {z_{D}}(t))= \langle (\eta_P \quat {\mu_D}-\eta_D\quat{\mu_P}+ \quat{\mu_P}\times \quat{\mu_D}),-\frac{1}{2}K \quat p_e\rangle\\=-K\frac{\langle \quat p_e,\quat p_e \rangle}{4}
    \label{eq:lypu_candidate_parts3}
\end{multline}
As $\frac{1}{2}\phi_e\text{sin}\left (\frac{1}{2}\phi_e \right ) \geq 0$ for $[-\pi,\pi]$,  then it stands that  $\dot{V_1}(\quat {z_{P}}(t))\leq -K\langle \quat n_e, \quat n_e \rangle $. Hence, 
\begin{equation}
    \dot V(\dq z(t) ) \leq  -K\langle \quat n_e, \quat n_e \rangle -K\frac{ \norm{\quat p_e}^2}{4} \leq 0. \label{eq:lypu_candidate2}
\end{equation}
As \eqref{eq:lypu_candidate2} demonstrates, $\dot V(\dq z(t) )$ is a negative definite. Therefore, we demonstrate that the system asymptotically stable in the sense of Lyapunov.

